First investigation of eclipsing binary KIC 9026766: analysis of light curve and periodic changes

Abstract We investigate a short-period W UMa binary KIC 9026766 with an orbital period of 0.2721278 days in the Kepler field of view. By using an automated q-search for the folded light curve and producing a synthetic light curve for this object based on the PHOEBE code, we calculate the fundamental stellar parameters. We also analyze the O-C curve of the primary minima. The orbital period changes can be attributed to the combination of an upward quadratic function and light-travel time effect due to a possible third body with a minimum mass of 0.029 solar mass and an orbital period of 972.5866 days. The relative luminosity of the primary and secondary eclipses (Min I Min II) is calculated. The periodogram of the residuals of the LTT effect, and Min I Min II show peaks with the same period of 0.8566 days. The background effect of two nearby stars on our target is the possible reason for this signal. By considering the amplitudes and periods of the remaining signals in the OC curve of minima, spot motion is possible.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

